Distorted Magnetic Flux Ropes within Interplanetary Coronal Mass Ejections

Magnetic flux ropes within interplanetary coronal mass ejections are often characterized as simplistic cylindrical or toroidal tubes with field lines that twist around the cylinder or torus axis. Recent multi-point observations suggest that the overall geometry of these large-scale structures may be significantly more complex, so that the contemporary modeling approaches would be, in some cases, insufficient to properly understand the global structure of any interplanetary coronal mass ejection. In an attempt to partially rectify this issue, we have developed a novel magnetic flux rope model that allows for the description of arbitrary distortions of the cross-section or deformation of the magnetic axis. The distorted magnetic flux rope model is a fully analytic flux rope model, that can be used to describe significantly more complex geometries and is numerically efficient enough to be used for large ensemble simulations. To demonstrate the usefulness of our model, we focus on a specific implementation of our model and apply it to an ICME event that was observed \textit{in situ} on 2023 April 23 at the L1 point by the Wind spacecraft and also by the STEREO-A spacecraft that was $10.2^\circ$ further east and $0.9^\circ$ south in heliographic coordinates. We demonstrate that our model can accurately reconstruct each observation individual and also gives a fair reconstruction of both events simultaneously using a multi-point reconstruction approach, which results in a geometry that is not fully constistent with a cylindrical or toroidal approximation.

==> old.tex <==
% The boundary surface of the flux rope, within the context of our coordinate system, can be implicitly defined by the isosurface for $\mu=1$, which by construction should be a flux surface. We further assume that all surfaces defined by a constant $\mu$ coordinate are flux surfaces. We can decompose the magnetic field vector in terms of components of our curvilinear coordinate system, so that $\vb*{B}(\mu,\nu,s)=\vb*{\epsilon}_i(\mu,\nu,s)B^i(\mu,\nu,s)$. The basis vectors have the property that $\vb*{\epsilon}_i\vb*{\epsilon}^j=\delta_i^j$, which allows us to construct the covariant $\mu$ basis vector using  $\vb*{\epsilon}^\mu = \left(\vb*{\epsilon}_\nu\cross\vb*{\epsilon}_s\right)g^{-\nicefrac{1}{2}}$. This vector also happens to point in the same direction as the surface normal vector  for the corresponding flux surface. From the constraint $\hat{\vb*{n}}\cdot\vb*{B}=0$, that must hold for any flux surface, it then automatically follows that $B^\mu=0$ everywhere. This property will allow us to simplify the model significantly, if we limit ourselves to working with the contravariant components of the magnetic field, which are $B^\nu$ and $B^s$.

% The flux rope model that we aim to develop will only describe an arbitrary flux rope as a snapshot in time. We do not care about deriving magnetohydrostatic solutions or about the time evolution. As a result we will omit any derivatives with respect to time. We start by writing down the three conditions that must be satisfied for any physically valid flux rope structure. By definition, when defining a flux rope as a twisted flux tube, any flux rope must at the same time also be a flux tube. Combining this with the fact that the magnetic field $\vb*{B}$ is a solenoid vector field we get following two basic constraints:
% \begin{eqnarray}
% \div \vb*{B}(\vb*{x}) &=& 0,\label{eq:bdnull}\\
% \vb*{\hat{n}}(\vb*{x})\cdot\vb*{B}(\vb*{x}) &=& 0,\label{eq:brnull}
% \end{eqnarray}
% where $\vb*{\hat{n}}(\vb*{x})$ describes the unit normal vector with respect to the outer boundary surface of the flux tube or rope. The constraint in Eq. \eqref{eq:brnull} can be used to define so-called flux surfaces, which must always be topological tori for a closed magnetic field configuration \adc. Given a well-behaved magnetic field structure, we assume that any point within our flux rope structure can be assigned to such a flux surface. This leads to a series of nested flux surfaces, which on the smaller end converge towards a line called the magnetic axis $\vb*{\gamma}$. Note that this is not necessarily the case, and we must explicitly exclude the existence of magnetic islands which would complicate our picture. Such structures are regularly seen in simulations \adc and play an important role in laboratory plasma physics \adc. 


% The often used third constraint, is that the flux rope should also be closed with respect to the current $\vb*{J}$, so that:
% \begin{eqnarray}
% \vb*{\hat{n}}(\vb*{x})\cdot\vb*{J}(\vb*{x}) = \vb*{\hat{n}}(\vb*{x})\cdot\left[ \curl\vb*{B}(\vb*{x})\right] = 0,\label{eq:jrnull}
% \end{eqnarray}
% where we make use of Ampere's law and disregard the time-varying electric field.
% 
% The standard approach for deriving most existing flux rope models starts by assuming that the flux rope either has a cylindrical or toroidal symmetry so that the constraints can be written in a simple and elegant form in their respective coordinate systems. The radial magnetic field and current, i.e. the component pointing directly away from the magnetic axis, is assumed to vanish everywhere and not only on the boundary so that one only needs to account for the axial and poloidal components. This implicitly assume that all flux surfaces are also concentric cylinders around the magnetic axis. The initially three dimensional problem is thus simplified to a single dimension and any physical quantity, such as the magnetic field vector $\vb*{B}$ or the current $\vb*{J}$, is only dependent on the distance to the magnetic axis. This then results in a class of solutions, where one can allow for different radial profiles and varying degrees force-freeness \citep[e.g.]{}{}. Illustrative examples of this approach can be followed in \add[ajw]{give nice examples}. In the general case, most of these simplifications can no longer be used and we have to allow for terms to vary along the magnetic axis and allow for non-zero radial magnetic fields as long as they do not directly violate the boundary conditions. In the following section, we will introduce what we call the ``distorted tubal coordinate system'', which is a further development of the coordinate system used in W22, which allows us to simplify the equations even when the radial magnetic field component is non-zero. While this coordinate system allows us to describe vastly more complex flux rope geometries, including all currently existing models, there are simple counter examples so that our model does not represent a general solution.

% %The solenoidal condition, stated in Eq. \eqref{eq:bdnull}, will unfortunately lead us to a non-analytical expression for the magnetic field components which cannot be simplified except in the cases where the cross-section geometry is given by a simple shape (e.g. circular). We will discuss the constraint from Eq. \eqref{eq:jrnull} afterwards in more detail as it can also be satisfied but only by imposing additional boundary conditions on the magnetic field.
% \add[]{}{more about curvilinear coordinate systems}In the rest of this manuscript, we will make use of standard Einstein notation, with upper and lower indices denoting contra- and covariant vectors respectively. Note that any basis vectors have the inverse convention. Most functions that depend on a single or multiple coordinates will be written in a very compact form, except when they are initially introduced, in order to keep the equations more readable.

% We use an approach that is some ways very similar to 

% The initial approach that we will use is largely equivalent to the approach that is used to construct coordinate systems in fusion-plasma physics \adc. The main difference is that our primary goal is to use a coordinate system that allows to easily describe distorted flux ropes. For the confinement plasma, it is important to find a magnetic field structure and a corresponding coordinate system that is stable over a long enough time scale. The structures we are interested in propagate from the Sun to Earth and beyond, they expand in size by multiple magnitudes, and are strongly influenced by the surrounding solar wind. It is thus very unlikely that the magnetic field configurations, that are largely force-free, are good descriptions 


% Figure \ref{fig:dt_example} shows an example of a distorted tubal flux rope as it can be described using our approach with a bent axis and varying cross-section shape. Using different expressions for $\mathcal{D}$ and $\Omega$, the possible cross-section shapes can take on many different forms. Taken to the extreme, $\Omega$ does not have to be bijective with respect to the coordinate $\nu$. This allows us to describe cross-section shapes with large dents, as is shown in Fig. \ref{fig:dt_example}b for $\mu=1$. The distorted cross-section also does not have to be self-similar with respect to the distance from the axis, so that we can describe shapes that are highly distorted only at the boundary but have circular symmetry near the magnetic axis.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[trim=50 0 50 25, clip,width=0.42\linewidth]{cs3d.pdf}
%     \includegraphics[trim=0 15 15 0, clip,width=0.45\linewidth]{cs.pdf}
%     \caption{Exemplary distorted tubal flux rope with a cross-section that varies over the axis. This particular example is largely circular symmetric at both ends and highly distorted at the center. \textit{Left}: Three dimensional representation with the cross-section highlighted at the center and the $\{\vb*{\hat{t}},\,\vb*{\hat{n}}_1,\,\vb*{\hat{n}}_2\}$ vectors in black, red and blue respectively. Shown flux surfaces are for $\mu=1$ and $\mu=0.5$. Boundary intersections of the flux rope with different $x-y$ planes are shown in magenta. \textit{Right}: Highlighted cross-section shown in a plane with three separate flux surface contours. We also show two circular symmetric contours for comparison that are thinner. The geometry of the cross-section is only distorted near the edge and is almost fully circular near the flux rope axis. For $\mu=1$, the cross-section shape is dented and the $\Omega$ function is not bijective with respect to the $\nu$ coordinate.} 
%     \label{fig:dt_example}
% \end{figure} 


% The relevant equations for both the magnetic field $\vb*{B}$,  the current density $\vb*{J}$, can be written as:

% Fortunately, there is no requirement to fully solve all of these equations because we are not interested in solving for specific current distributions. For now, let us focus on finding expressions that only satisfy Eq. \eqref{eq:gauss_law}, for which an example can be easily found that takes the following form:
% \begin{eqnarray}
% B^\nu=\frac{\left(\chi + \partial_s H\right)(\mu,s)}{\g},\label{eq:b_nu}\\
% B^s=\frac{\left(\xi + \partial_\nu H\right)(\mu,\nu)}{\g},\label{eq:b_s}
% \end{eqnarray}
% where $\left(\chi + \partial_s H\right)$ and $\left(\xi + \partial_\nu H\right)$ are functions that appear as integration constants with two variables. At first glance, this solution appears surprisingly simple, but it is important to note that the entire complexity is obfuscated by our coordinate system. 


% \subsection{Boundary Conditions}

% Before we continue, we will take a closer look at boundary conditions that will give us more specific information or constraints on the functions that we use. We assume that our flux rope is closed, and that it topologically corresponds to a torus. From practical considerations within the context of heliospheric structures, it does not always make sense to describe the full structure, and we will therefore allow violations of the condition that the magnetic field, and thus all functions that we use to define the, are periodic with respect to the $s$-coordinate. It should also be abundantly clear that the magnetic field and all functions should be period with respect to the $\nu$-coordinate. The only remaining boundaries that we need to check more carefully, are thus the magnetic axis at $\mu=0$, and the boundary flux surface at $\mu=1$.

% , the relevant areas that we need to check is the magnetic axis itself at $\mu=0$ and the outer flux rope boundary at $\mu=1$. We will start with the ``inner'' boundary at 

% From the way we constructed our coordinate system. It is clear that $\mathcal{D},\,\partial_\nu\mathcal{D}$ and $\partial_s\mathcal{D}$ must vanish at $\mu=0$. \n{more stuff for $\mu=0$}.

% The constraints for $\mu=1$ turn out to be slightly more complicated. Both the magnetic field vector, and the current density can take any value as long as they lie on the boundary flux surface. By construction, we are guaranteed that $B^\mu=0$, but we have made no such constraint for $J^\mu$, which we can fully write out as:
% \begin{equation}
% J^\mu=\frac{1}{\mu_0\g}\left[\right]
% \end{equation}
% \n{more about current problem near boundary}

% \section{Applications}

% Exemplary AEM family with parameters $(\alpha,\beta,\delta,\epsilon,\sigma)$:
% \begin{eqnarray}
% \vb*{\gamma}&=&\lbrace 1 - \cos(2 \pi s),\,\sin(2 \pi s) \sin^\alpha(\pi s),\,\beta \sin^4(\pi s)\sin(\epsilon\,\pi s)\rbrace,\\
% \mathcal{D}&=&r\sigma \left[1+(\delta - 1)\cos^4(2\pi s)\right]
% \end{eqnarray}

% \subsection{Re-imagining Empirical Models}

